Real-Time Anomaly Detection and Reactive Planning with Large Language Models

Foundation models, e.g., large language models (LLMs), trained on internet-scale data possess zero-shot generalization capabilities that make them a promising technology towards detecting and mitigating out-of-distribution failure modes of robotic systems. Fully realizing this promise, however, poses two challenges: (i) mitigating the considerable computational expense of these models such that they may be applied online, and (ii) incorporating their judgement regarding potential anomalies into a safe control framework. In this work, we present a two-stage reasoning framework: First is a fast binary anomaly classifier that analyzes observations in an LLM embedding space, which may then trigger a slower fallback selection stage that utilizes the reasoning capabilities of generative LLMs. These stages correspond to branch points in a model predictive control strategy that maintains the joint feasibility of continuing along various fallback plans to account for the slow reasoner's latency as soon as an anomaly is detected, thus ensuring safety. We show that our fast anomaly classifier outperforms autoregressive reasoning with state-of-the-art GPT models, even when instantiated with relatively small language models. This enables our runtime monitor to improve the trustworthiness of dynamic robotic systems, such as quadrotors or autonomous vehicles, under resource and time constraints. Videos illustrating our approach in both simulation and real-world experiments are available on this project page: https://sites.google.com/view/aesop-llm.

==> rebuttal.tex <==
\section{Author Response}
Here, we include detailed responses to the reviewers' comments and an account of all the changes that we have made in the revised version of the paper, which can be found from \textbf{page 4 onwards} in this document. We have structured this list in separate blocks, corresponding to the suggestions made by the AC and reviewers. Comments and suggestions by the AC and reviewers are highlighted in {\color{red} red}. To help reviewers identify our revisions, sections of the paper that were added or modified in this revision are highlighted in {\color{blue} blue}, both in the body of the paper and in this author response. Text that was present in the initial submission is marked in {\color{magenta} magenta} in this statement of revision.
We would like to thank all the reviewers for their thoughtful and constructive remarks.

\subsection{Response to AC}
We thank the AC for their constructive feedback, the opportunity to revise the paper, and noting that our manuscript is \inlinecomment{well-written} and addresses a problem that is \inlinecomment{essential for practical applications}. We have addressed the areas for clarification and stated limitations to the best of our ability, most notably:
\begin{enumerate}
    \item \textbf{Hardware experiment:} We have implemented our approach on a quadrotor hardware platform to validate the efficacy of our method beyond simulation, which we document in \inlineedit{\cref{sec:exps-hardware}, \cref{app:hardware}, and the video in the supplementary material}. These experiments show that we can effectively leverage LLMs and embedding models for reactive control on real-robot hardware using compute platforms designed for embedded systems.
    \item \textbf{Theoretical and experimental clarifications:} We have added clarifying statements and a description of notation throughout the body of the paper (and in \cref{ap:glos}), which we hope improves the clarity and strength of our theoretical result, methodology (e.g., handling of anomalies that do not require intervention), and experimental setup.
    \item \textbf{Future work:} We have revised the conclusion of our paper to include a discussion on future work related to some of the comments raised by the reviewers. In particular, while our work clearly represents an improvement in accounting for LLM latency in an agile control stack, future work should investigate remaining practical challenges like handling the rare instances where an LLM produces an incoherent response.
\end{enumerate}

\subsection{Response to Reviewer JEHY}
We thank the reviewer for their insightful comments and appreciation of our manuscript. The suggestions the reviewer made have helped us significantly improve the clarity of our manuscript. We respond to specific comments below:
\comment{Using small \dots large delays.}
We agree that computational considerations are paramount for agile robot hardware, which has motivated much of our work: As noted by the reviewer, we can leverage small embedding models that run in real-time on relatively cheap hardware (e.g., an Nvidia Jetson) to account for the latencies associated with (cloud querying) chain-of-thought generation with LLMs. To further emphasize this point, we have now implemented our approach on a quadrotor hardware testbed (described in \inlineedit{\cref{sec:exps-hardware}}), where we show our method's real-time feasibility. 

Even though running GPU-enabled platforms like the Nvidia Jetson on small systems is feasible and becoming increasingly common (e.g., see \cite{kaufmann2023champion}), we agree with the reviewer that the power consumption of such systems can pose challenges. As has been the trend in recent years, we expect future hardware developments to increase the efficiency of such systems. Moreover, our methodology could further benefit system efficiency when the slow-reasoning process runs on-device since we only query the generative LLM when we truly require its capabilities. 

\comment{Clarifications: Should \dots always be $-1$.}
We thank the reviewer for noting this small oversight in our manuscript. The reviewer is correct in noting that we compute similarity scores in a leave-one-out fashion to calibrate the threshold, otherwise the nominal similarity scores are always $-1$. We have corrected \inlineedit{equation \cref{eq:emp-quantile}} in the revised manuscript and added the following sentence for clarity: 
% \edit{Note that for nominal embeddings we must compute the anomaly score $\s$ in a leave-one-out fashion, since $\s(\e_i ; \calD_e) = -1$ for $\e_i \in \calD_e$.}
\edit{Note that for nominal embeddings, we must compute the anomaly score $\s$ in a leave-one-out fashion, since $\s(\e_i ; \calD_e) = -1$ for $\e_i \in \calD_e$.}

\inlinecomment{Typos: \dots} We have fixed the noted typos in the revised manuscript, and thank the reviewer for pointing them out.
\subsection{Response to Reviewer 1APW}
We thank the reviewer for their positive comments, in particular for noting that our application is \inlinecomment{interesting and novel}, that our experiments are \inlinecomment{diverse and thorough}, and tackles the \inlinecomment{practical aspect of inference time for LLMs}. We have also made several changes to our manuscript, which we hope address the noted limitations and feedback for clarification:

\comment{Experiments were \dots synthetic environments.}

We agree with the reviewer that a hardware demonstration would strengthen our manuscript. Thus, we have implemented our approach on a quadrotor hardware platform to validate the efficacy of our method, which we document in \inlineedit{\cref{sec:exps-hardware} and the videos included in the supplementary material.} We believe these experiments further showcase 1) the efficacy of our approach, 2) its real-world practicality, and 3) its real-time feasibility, supporting the thesis that we can effectively leverage LLMs and embedding models for reactive control on real-robot hardware using compute platforms designed for embedded systems.

\comment{Theorem 1 \dots fairly trivially.}
% \chris{See below for shortened response.}
% We agree with the reviewer that \cref{thm:safety} resembles a typical recursive feasibility argument from the MPC literature (e.g., see \cite{BorrelliBemporadEtAl2017}) that is a direct consequence of the careful construction of Algorithm \ref{alg:safe-mpc}. While, as the reviewer notes, the closed-loop properties that \cref{thm:safety} establishes are intuitive, we still include the theorem for two reasons: 1) Even though the properties of our algorithm are intuitive, we view the impact on the length and flow of the paper as minimal (since the proof is in the appendix) and include it for the sake of completeness. \cref{thm:safety} formally establishes the soundness of Algorithm \ref{alg:safe-mpc} and our design choices in the MPC \cref{eq:modification-mpc}, which is typical in the MPC literature. 2) While \cref{thm:safety} establishes properties that are intuitive for readers familiar with canonical MPC theory and recursive feasibility results (as in e.g., \cite{BorrelliBemporadEtAl2017}), we choose to include the theorem to make the properties of our algorithm obvious to readers who are less familiar with MPC results. We hope this ensures a minimal barrier to entry and improves clarity for readers who are not familiar with classical MPC arguments.
% We agree with the reviewer that \cref{thm:safety} resembles a typical recursive feasibility argument from the MPC literature (e.g., see \cite{BorrelliBemporadEtAl2017}) that is a direct consequence of the careful construction of Algorithm \ref{alg:safe-mpc}. While, as the reviewer notes, the closed-loop properties that \cref{thm:safety} establishes are intuitive, we still include the theorem for two reasons: 1) Even though the properties of our algorithm are intuitive, we view the impact on the length and flow of the paper as minimal (since the proof is in the appendix) and include it for the sake of completeness. \cref{thm:safety} formally establishes the soundness of Algorithm \ref{alg:safe-mpc} and our design choices in the MPC \cref{eq:modification-mpc}, which is typical in the MPC literature. 2) While \cref{thm:safety} establishes properties that are intuitive for readers familiar with canonical MPC theory and recursive feasibility results (as in e.g., \cite{BorrelliBemporadEtAl2017}), we choose to include the theorem to make the properties of our algorithm obvious to readers who are less familiar with MPC results. We hope this ensures a minimal barrier to entry and improves clarity for readers who are not familiar with classical MPC arguments.

We agree with the reviewer that \cref{thm:safety} resembles a typical recursive feasibility argument from the MPC literature, (e.g., see \cite{BorrelliBemporadEtAl2017}), i.e., that initial feasibility of the MPC at $t=0$ inductively implies feasibility and reachability of the recovery sets for all $t > 0$ for the closed-loop system. This is a direct consequence of the careful construction of Algorithm \ref{alg:safe-mpc}. While the closed-loop properties that \cref{thm:safety} establishes are indeed intuitive, we choose to include the theorem for two reasons: 1) To make the properties of our algorithm obvious to readers who are less familiar with canonical MPC theory and recursive feasibility results (as in e.g., \cite{BorrelliBemporadEtAl2017}), providing clarity and lowering the barrier to entry. 2) We view the impact on the length and flow of the paper as minimal (since the proof is in the appendix) and include it for the sake of completeness. We have also added the following phrase to the body of the paper to clarify the theorem, which we hope helps alleviate the reviewer's comment:
 \edit{ which guarantees that we reach the recovery set chosen by the slow reasoner within at most $T+1$ timesteps after detecting an anomaly:}
% \cref{thm:safety} formally establishes the soundness of Algorithm \ref{alg:safe-mpc} and our design choices in the MPC \cref{eq:modification-mpc}, which is typical in the MPC literature. 

% \chris{Despite the reviewer being incorrect in their assumptions, we should consider removing this point avoid drawing unnecessary attention.}

% We would also like to note that we do not assume that \inlinecomment{there always exist reachable recovery sets}, nor do we always assume the MPC is feasible. We only assume that there exists some subset of recovery sets for which the MPC is feasible at $t=0$. Algorithm \ref{alg:safe-mpc} then ensures that there always exist reachable recovery sets for all $t>0$ by design. \rohan{optional: We have added the following clarifying phrase to the body surrounding the theorem }

\subsection{Response to Reviewer EWSP}
We would like to thank the reviewer for their insightful comments and engaging so thoroughly with the ideas in our manuscript. We have made several changes to the manuscript in response to these comments, which we detail below:

\comment{From what I \dots a decision.}
We agree with the reviewer that cloud APIs could experience connectivity issues and that even when using a local model, the model could unexpectedly produce a very long outputs in rare cases, thereby pushing the latency of the slow reasoner beyond the limit of $K$ timesteps that we assume in the control design. We have made several changes to make this point more prominent in the paper and discuss our algorithmic rationale here.    

We use a fixed $K$ for two reasons: 1) It is the most natural way to account for latency in the control design. 2) $K$ should represent an upper bound: Our algorithm guarantees safety as long as the response time is less than K time steps. As we wrote in the original manuscript (last paragraph of \cref{sec:fast-and-slow}) 
\original{It is usually uncomplicated to identify the value of $K$ in practice, since we prompt the model to adhere to a strict output template that tends to stabilize the length of the output generations. Alternatively, a simple field-test should be sufficient to identify upper bounds on network latency.}

We have found that with state-of-the-art LLMs, response lengths are mostly consistent and hardly violate expected output formats, and therefore we gravitated towards a simple approach with a fixed latency $K$. In the revised paper, we have also implemented our framework in closed-loop on a quadrotor hardware platform \inlineedit{(see \cref{sec:exps-hardware})}, where we did not experience issues due to our choice of $K$. To substantiate this point, we have added an analysis of the slow-reasoner's query latency in \inlineedit{\cref{app:hardware}} where we plot a histogram of GPT-3.5 query latencies (which we used for the hardware experiments) and discuss our choice of $K$. To be more precise in our claims, we have also modified the above quote to 
\edit{\dots Alternatively, as we describe in \cref{sec:exps-hardware} and \cref{app:hardware}, a simple field-test can be sufficient to identify an upper bound on typical network latency.}

Nevertheless, we agree that it is challenging to make hard guarantees on LLM latencies and response lengths. We think this presents an excellent opportunity for future work, as we discuss in the updated conclusion:

\edit{For example, the impact of LLM inference latencies could be reduced by devising methods to constrain generative reasoning to a fixed word budget, or by using intermediate generations to inform decision-making during the generation process.}

% Can we devise methods to guarantee LLMs adhere to e.g., token count limits/inference times? Or, would it be possible to make intermediate conclusions from partial outputs throughout the generation process? We have added a discussion of this point to the future works section of the conclusion. Future work could also investigate variations of our MPC planner that are amenable to random, perhaps unbounded, response times. We did not do so here, as we wanted to guarantee the robot reaches a recovery region within T timesteps of an anomaly occurring. 
 

 
\comment{It seems \dots the paper.}
We agree that control strategies that are amenable to random and perhaps unbounded response times represent an interesting direction for future work, and we agree that a backup scheme to select a fallback upon model timeout makes sense as a first step. We consider this a topic for future work, as it is not obvious how to devise such a backup scheme. In particular, it is not the case that all recovery strategies are equally safety-preserving in all circumstances. For example, if the VTOL air taxi has options \{``hover in place”, ``land in a field”\}, and the anomaly is ``a large swarm of birds heading towards the drone,” it would be unsafe to hover in place. Therefore, the LLM’s reasoning is necessary at present, as it is unclear to us how one would make an assessment for any out-of-distribution scenario with another method (like selecting a random fallback). We have included the following comment in the conlcusion of the paper in the revision: 
\edit{Further analysis is required on the \textit{correctness} of fallback plans selected by the LLM, and whether fallbacks can be programmatically determined upon latency timeout.}

\comment{The ``slow \dots synthetic domains.}
% \chris{Shortened version below.}
% We originally did not include evaluations of the other synthetic domains due to space constraints and API query limits. However, we agree with the reviewer that these evaluations would improve the completeness of the experiments in the manuscript. We have added a full table across all synthetic environments in \rohan{todo: in appendix or main body?}.

% We thank the reviewer for their suggestion and have extended the evaluation of the slow reasoner across all three synthetic domains (including an additional model, GPT-3.5 Turbo) for completeness. The full results table can be found in \rohan{todo: in appendix or main body?}.

We thank the reviewer for their suggestion and have extended the evaluation of the slow reasoner to the manipulation domain (including an additional model, GPT-3.5 Turbo). 
The result can be found in \cref{appx:anomaly-assessment}.
We note that the CARLA experiment (\cref{sec:exps-ablation}) already evaluates the slow reasoner in an autonomous vehicle setting, which extends beyond the synthetic domains by interfacing the LLM with an onboard perception pipeline.


\comment{The third \dots detected anomalies.}
 We agree that it would have been preferred to generate scenarios that are anomalous but not safety critical for CARLA. However, for this experiment we used a dataset that originated from a related paper \cite{elhafsi2023}, where all anomalies were set up specifically to confuse an AV stack. These anomalies are careful recreations of documented real-world failure modes of current self-driving vehicles, whereas we are not aware of publicly documented ``interesting anomalies'' that did not confuse real self-driving vehicles. Hence, we were unfortunately not able to augment this existing dataset. However, we still consider the combination of 1) the additional hardware experiment \inlineedit{(see \cref{sec:exps-hardware} and the supplementary videos)}, 2) our synthetic evaluations, 3) closed-loop simulations, and 4) the CARLA evaluation on existing data as a diverse enough suite of experiments to fully validate our proposed methodology.

\comment{When describing \dots that process.}
% \chris{Here, we are explaining when we don't need to. Just thank the reviewer for highlighting an area to improve clarity and state that improvement. Made this change below.}

% Our intent with this statement was to explain intuitively what the metric in the equation encodes: The max over similarities implies that we retrieve the most similar observation from the prior experience data, and then use the similarity score associated with that observation. In Python code, this simply corresponds to \texttt{- np.max(embedding\_matrix @ query)}, where the embedding matrix and query vector are (row-wise) normalized. We have modified this sentence to
We thank the reviewer for highlighting the need clarification. We have have modified this sentence accordingly to
\edit{For example, the simplest metric uses the maximum cosine similarity with respect to samples in the prior experience cache, 
\begin{equation*}
    \s(\e_t; \calD_e) := - \max_{\e_i \in \calD_{e}} {\frac{\e_i^T \e_t}{\|\e_i\|\|\e_t\|}},
\end{equation*}
which in effect retrieves the most similar prior experience from $\calD_e$ to construct the score. Intuitively, this approach measures whether anything similar to the current observation has been seen before.}
 
The computational cost of this procedure (which amounts to a single matrix-vector multiplication) was negligible on all of the datasets we considered. We have added the footnote
\edit{In all our experiments, the computational cost of computing similarity scores with given embeddings was negligible compared to model inference times.}
in our discussion of compute latency in \cref{sec:exps-drone}.

\comment{In the case \dots could help.}
We do not currently handle this, the anomaly detector would trigger again. On-line continual learning/adaptation based on the delayed outputs of the LLM is absolutely an interesting direction for future work, and could also be used to dynamically adjust the false positive/negative rates! We have added the sentence 
\edit{Finally, continual learning based on the delayed anomaly assessment of the generative reasoner can be used to avoid triggering non-safety-critical anomalies a second time.}
to the discussion of future work in the conclusion in response to the reviewer's comment.

\comment{From what \dots equation 2.}
 FPR and TPR refer to the false positive rate (number of nominal examples that are detected as anomalous) and true positive rate (number of correctly detected anomalies). We have added clarifications of these acronyms and a note explaining what the bolded numbers mean to the table captions. In addition we have added the sentence
 \edit{\dots i.e., the smallest value of $q$ that upper bounds at least $\alpha N$ nominal samples. Determining the threshold $\tau$ using \dots}
 to clarify the variables in equation \cref{eq:emp-quantile} and 
 \edit{Here, the notation $\x^i_{t+k|t}$ indicates the predicted value of variable $\x$ at time $t+k$ computed at time $t$ for each trajectory $i \in \calY \cup \{0\}$.}
 to clarify the notation in the MPC problem \cref{eq:modification-mpc}.
 Furthermore, we include a detailed glossary that explains all notation and defines all symbols used in this paper to \inlineedit{\cref{ap:glos}} and reference it in the introduction of the paper. We hope this improves the clarity of the paper and alleviates the reviewer's concerns.


